Free-T2M: Robust Text-to-Motion Generation for Humanoid Robots via Frequency-Domain

Enabling humanoid robots to synthesize complex, physically coherent motions from natural language commands is a cornerstone of autonomous robotics and human-robot interaction. While diffusion models have shown promise in this text-to-motion (T2M) task, they often generate semantically flawed or unstable motions, limiting their applicability to real-world robots. This paper reframes the T2M problem from a frequency-domain perspective, revealing that the generative process mirrors a hierarchical control paradigm. We identify two critical phases: a semantic planning stage, where low-frequency components establish the global motion trajectory, and a fine-grained execution stage, where high-frequency details refine the movement. To address the distinct challenges of each phase, we introduce Frequency enhanced text-to-motion (Free-T2M), a framework incorporating stage-specific frequency-domain consistency alignment. We design a frequency-domain temporal-adaptive module to modulate the alignment effects of different frequency bands. These designs enforce robustness in the foundational semantic plan and enhance the accuracy of detailed execution. Extensive experiments show our method dramatically improves motion quality and semantic correctness. Notably, when applied to the StableMoFusion baseline, Free-T2M reduces the FID from 0.152 to 0.060, establishing a new state-of-the-art within diffusion architectures. These findings underscore the critical role of frequency-domain insights for generating robust and reliable motions, paving the way for more intuitive natural language control of robots.

==> tab/ablation_stable.tex <==
% \begin{table*}[htbp]
% \centering
% \resizebox{0.8\textwidth}{!}{%
% \begin{tabular}{lccccc}
% \hline
% \textbf{Method} & \textbf{FID $\downarrow$} & \multicolumn{3}{c}{\textbf{R-Precision $\uparrow$}} & \textbf{Diversity $\rightarrow$} \\ \cline{3-5}
%  &  & \textbf{top1} & \textbf{top2} & \textbf{top3} \\ \hline


% \(\mathcal{L_\text{LF}} + \mathcal{L}_\text{S}\)    
%                               & $\mathbf{0.261^{\pm0.043}}$ & $\mathbf{0.466^{\pm0.008}}$ & $\mathbf{0.657^{\pm0.007}}$ & $\mathbf{0.757^{\pm0.005}}$ & $9.666^{\pm0.078}$ \\ 

% \(\mathcal{L}_\text{LF}\) only        & $0.444^{\pm0.003}$ & $0.456^{\pm0.004}$ & $0.652^{\pm0.001}$ & $0.759^{\pm0.001}$ & $9.637^{\pm0.005}$ \\ 

% \(\mathcal{L}_\text{S}\) only        & $0.731^{\pm0.066}$ & $0.4305^{\pm0.007}$ & $0.619^{\pm0.006}$ & $0.722^{\pm0.006}$ & $\mathbf{9.464^{\pm0.076}}$ \\ \hline
% \end{tabular}%
% }
% \caption{Ablation experiment results of MDM$_{50steps}$ for \(\mathcal{L}_\text{LF}\) and \(\mathcal{L}_\text{S}\) on the HumanML3D test set. Bold indicates the best result.}
% \label{table:ablation_results}
% \end{table*}

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccc}
\hline
\textbf{Method} & \textbf{FID $\downarrow$} & \multicolumn{3}{c}{\textbf{R-Precision $\uparrow$}}  \\ \cline{3-5}
 &  & \textbf{top1} & \textbf{top2} & \textbf{top3} \\ \hline


\(\mathcal{L_\text{LF}} + \mathcal{L}_\text{S}\)    
                              & $\mathbf{0.051^{\pm0.002}}$ & $\mathbf{0.520^{\pm0.013}}$ & $\mathbf{0.707^{\pm0.003}}$ & $\mathbf{0.803^{\pm0.006}}$  \\ 

\(\mathcal{L}_\text{LF}\) only        & $0.172^{\pm0.007}$ & $0.538^{\pm0.004}$ & $0.734^{\pm0.072}$ & $0.820^{\pm0.005}$  \\ 

\(\mathcal{L}_\text{S}\) only        & $0.511^{\pm0.066}$ & $0.539^{\pm0.031}$ & $0.731^{\pm0.005}$ & $0.819^{\pm0.043}$  \\ \hline
\end{tabular}%
}
\caption{Ablation experiment results of StableMofFusion for \(\mathcal{L}_\text{LF}\) and \(\mathcal{L}_\text{S}\) on the HumanML3D test set. Bold indicates the best result.}
\label{table:ablation_results}
% \vspace{0.3cm}
\end{table}

==> tab/efficiency.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{ccccc}
        \hline
        Time &MDM & Free-MDM & StableMoFusion & Free-StableMoFusion  \\
        \hline
        Training time & 72h & 84h & 96h & 108h \\
        Inference time & 0.045s & 0.045s & 0.036s & 0.036s \\

        \hline
    \end{tabular}
    \caption{Training Time and Inference Time: We conducted our experiments on an NVIDIA 3090 GPU. Training Time refers to the time required for MDM to complete 600,000 steps and StableMoFusion to complete 200,000 steps. Inference Time represents the average time needed by each of the four models to generate 200 samples.}
    \label{tab:training_inference_time}
\end{table}

==> tab/eval_num.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[ht]
\centering
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{lclll}
\hline
Method                   & \multicolumn{1}{l}{Num} & Top-1 & Top-2 & Top-3 \\ \hline
Real                     & \multirow{3}{*}{8}      &0.771       & 0.912      &  0.962     \\
Free-StableMoFusion      &                         & \textbf{0.775}      & \textbf{0.923}      & \textbf{0.969}      \\
StableMoFusion(baseline) &                         &   0.753    & 0.909      & 0.962      \\ \hline
Real                     & \multirow{3}{*}{16}     &  0.646     &  0.820     & 0.900      \\
Free-StableMoFusion      &                         &  \textbf{0.657}     & \textbf{0.841}      & \textbf{0.913}      \\
StableMoFusion(baseline) &                         & 0.634      & 0.816      & 0.892      \\ \hline
Real                     & \multirow{3}{*}{32}     &0.511       &  0.703     &  0.797     \\
Free-StableMoFusion      &                         & \textbf{0.520}      & \textbf{0.707}      & \textbf{0.803}      \\
StableMoFusion(baseline) &                         & 0.499      & 0.681      &0.779       \\ \hline
Real                     & \multirow{3}{*}{64}     &   0.374      &  0.560     & 0.672      \\
Free-StableMoFusion      &                         & \textbf{0.394}      &  \textbf{0.566}     &   \textbf{0.678}    \\
StableMoFusion(baseline) &                         &  0.378      &  0.550     & 0.647      \\ \hline

\end{tabular}%

}

\caption{R-Precision Results with Different Numbers of Sampled Texts. Our method achieves higher accuracy than the baseline across all sampling sizes, further demonstrating its ability to improve semantic consistency in generated results.}
\label{table:sample}
\end{table}


% Real                     & \multirow{3}{*}{128}    &       &       &       \\
% Free-StableMoFusion      &                         &       &       &       \\
% StableMoFusion(baseline) &                         &       &       &       \\ \hline

==> tab/fintune.tex <==
% \begin{table*}[htbp]
% \centering
% \resizebox{0.8\textwidth}{!}{%
% \begin{tabular}{lccccc}
% \hline
% \textbf{Method} & \textbf{FID $\downarrow$} & \multicolumn{3}{c}{\textbf{R-Precision $\uparrow$}} & \textbf{Diversity $\rightarrow$} \\ \cline{3-5}
%  &  & \textbf{top1} & \textbf{top2} & \textbf{top3} \\ \hline


% \(\mathcal{L_\text{LF}} + \mathcal{L}_\text{S}\)    
%                               & $\mathbf{0.261^{\pm0.043}}$ & $\mathbf{0.466^{\pm0.008}}$ & $\mathbf{0.657^{\pm0.007}}$ & $\mathbf{0.757^{\pm0.005}}$ & $9.666^{\pm0.078}$ \\ 

% \(\mathcal{L}_\text{LF}\) only        & $0.444^{\pm0.003}$ & $0.456^{\pm0.004}$ & $0.652^{\pm0.001}$ & $0.759^{\pm0.001}$ & $9.637^{\pm0.005}$ \\ 

% \(\mathcal{L}_\text{S}\) only        & $0.731^{\pm0.066}$ & $0.4305^{\pm0.007}$ & $0.619^{\pm0.006}$ & $0.722^{\pm0.006}$ & $\mathbf{9.464^{\pm0.076}}$ \\ \hline
% \end{tabular}%
% }
% \caption{Ablation experiment results of MDM$_{50steps}$ for \(\mathcal{L}_\text{LF}\) and \(\mathcal{L}_\text{S}\) on the HumanML3D test set. Bold indicates the best result.}
% \label{table:ablation_results}
% \end{table*}

\begin{table}[t]
\centering
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{lcccc}
\hline
\textbf{Method} & \textbf{FID $\downarrow$} & \multicolumn{3}{c}{\textbf{R-Precision $\uparrow$}}  \\ \cline{3-5}
 &  & \textbf{top1} & \textbf{top2} & \textbf{top3} \\ \hline
StableMoFusion (Baseline)& $0.189^{\pm0.003}$ & $0.499^{\pm0.004}$ & $0.680^{\pm0.006}$ & $0.779^{\pm0.007}$  \\ 
Free-StableMoFusion (Training)  & $\mathbf{0.051^{\pm0.002}}$ & $0.520^{\pm0.013}$ &$0.707^{\pm0.003}$ & $0.803^{\pm0.006}$ \\
Free-StableMoFusion (Fine-tuning)  
                              & $0.091^{\pm0.011}$ & $\mathbf{0.535^{\pm0.004}}$ & $\mathbf{0.728^{\pm0.041}}$ & $\mathbf{0.819^{\pm0.002}}$    \\ \hline
\end{tabular}%
}
\caption{Different training approaches for StableMoFusion: Fine-tuning the existing model using Free-T2M is more efficient and effective.}
\label{table:fine-tuning}

\end{table}

==> tab/high_frequency_loss.tex <==
% ---> [ground truth] R_precision: (top 1): 0.3815 (top 2): 0.5655 (top 3): 0.6697 
% ---> [text2motion] Matching Score: 5.3371
% ---> [text2motion] R_precision: (top 1): 0.1291 (top 2): 0.2240 (top 3): 0.3090 
% ---> [ground truth] FID: 0.0024
% ---> [text2motion] FID: 11.5805
% ---> [ground truth] Diversity: 9.0876
% ---> [text2motion] Diversity: 9.1501
% ---> [text2motion] Multimodality: 0.7584 这个


\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccc}
\hline
\textbf{Method} & \textbf{FID $\downarrow$} & \multicolumn{3}{c}{\textbf{R-Precision $\uparrow$}}  \\ \cline{3-5}
 &  & \textbf{top1} & \textbf{top2} & \textbf{top3} \\ \hline
StableMoFusion (Baseline)& $0.189^{\pm0.003}$ & $0.499^{\pm0.004}$ & $0.680^{\pm0.006}$ & $0.779^{\pm0.007}$  \\ 
Free-StableMoFusion (our)   & $0.051^{\pm0.002}$ & $0.520^{\pm0.013}$ &$0.707^{\pm0.003}$ & $0.803^{\pm0.006}$ \\
StableMoFusion ($L_h$)  
                             & $11.581^{\pm0.002}$  & $0.129^{\pm0.011}$ & $0.224^{\pm0.004}$ & $0.309^{\pm0.041}$     \\ \hline
\end{tabular}%
}
\caption{High Frequency Consistency Loss Ablation Study. When directly aligning high-frequency information, the sparsity of motion high-frequency data and its dependency on low-frequency information can lead to training failure.}
\label{table:high_frequency_loss}
\vspace{-0.5cm}
\end{table}


==> tab/humaneval.tex <==

\begin{table}[ht]
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{lll}
\hline
Method              & ACC   & Preference   \\\hline
MDM                 & 0.580 & 0.412 \\
MDM(ours)            & $\mathbf{0.650}$ & $\mathbf{0.588}$ \\
StableMoFusion      & 0.644 & 0.384 \\
StableMoFusion(ours) & $\mathbf{0.724}$ & $\mathbf{0.616}$ \\\hline
\end{tabular}}
\label{human_eval}
\caption{Human Evaluation Results. We randomly sampled 100 test texts for manual evaluation of correctness and user preference. The results demonstrate that our method improves model accuracy and garners higher user preference.}

\end{table}

==> tab/kit.tex <==
% \begin{table*}[htbp]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llccccc}
% \hline
% \textbf{Method} &Venue & \textbf{FID $\downarrow$} & \multicolumn{3}{c}{\textbf{R-Precision $\uparrow$}} & \textbf{Diversity $\rightarrow$} \\ \cline{4-6}
%  & &  & \textbf{top1} & \textbf{top2} & \textbf{top3} \\ \hline
% Real & & $0.031^{\pm0.004}$ & $0.424^{\pm0.005}$ & $0.649^{\pm0.006}$ & $0.779^{\pm0.006}$ & $11.08^{\pm0.097}$ \\

% MLD \cite{MLD}& CVPR 2023 &$0.404^{\pm0.027}$ & $0.390^{\pm0.008}$ & $0.609^{\pm0.008}$ & $3.204^{\pm0.027}$ & $10.80^{\pm0.117}$ \\

% ReMoDiffuse \cite{remodiffuse} & ICCV 2023&$\textcolor{blue}{$0.155^{\pm0.006}$} & $0.427^{\pm0.014}$ & $0.641^{\pm0.004}$ & $0.765^{\pm0.055}$ & $10.80^{\pm0.105}$ \\
% MotionDiffuse \cite{motiondiffuse}&TPAMI 2024 & $1.954^{\pm0.062}$ & $0.417^{\pm0.004}$ & $0.621^{\pm0.004}$ & $0.739^{\pm0.004}$ & $11.100^{\pm0.163}$ \\
% % MotionLCM \cite{motionlcm} &ECCV 2024& 0.467^{ \pm 0.012} &$0.502^{\pm0.003}$& \textcolor{blue}{$0.701^{\pm 0.002}$} & \textcolor{red}{$0.803^{\pm 0.002}$}  &$9.3610^{\pm 0.660}$\\
% T2M-GPT \cite{T2M-GPT}& CVPR 2023 &
% $0.514^{\pm0.029}$ & $0.416^{\pm0.006}$ & $0.627^{\pm0.006}$ & $0.745^{\pm0.006}$ & $10.921^{\pm0.108}$\\

% MDM_{50steps}(baseline) \cite{MDM}&ICLR 2023 & $0.497^{\pm0.021}$ & $0.164^{\pm0.004}$ & $0.291^{\pm0.004}$ & $0.396^{\pm0.004}$ & $10.847^{\pm0.109}$ \\ 

% MDM_{1000steps}(baseline) \cite{MDM}&ICLR 2023 & $0.556^{\pm0.0698}$ & $0.322^{\pm0.019}$ & $0.431^{\pm0.013}$ & $0.698^{\pm0.052}$ & $10.73^{\pm0.201}$ \\

% StableMoFusion (baseline) \cite{stablemofusion} & ACM MM 2024& $0.258^{\pm0.029}$ & \textcolor{red}{$0.445^{\pm0.006}$} & \textcolor{blue}{$0.660^{\pm0.005}$} & \textcolor{blue}{$0.782^{\pm0.004}$} & \textcolor{red}{$10.936^{\pm0.077}$} \\ \hline

% Free-MDM_{50steps}(Ours) &- & $0.401^{\pm0.033}$ & $0.382^{\pm0.006}$ & $0.587^{\pm0.006}$ & $0.707^{\pm0.007}$ & $10.733^{\pm0.102}$ \\ 

% Free-MDM_{1000steps}(Ours) &-& $0.529^{\pm0.036}$ & $0.377^{\pm0.004}$ & $0.579^{\pm0.007}$ & $0.705^{\pm0.006}$ & $10.826^{\pm0.117}$ \\ 

% Free-StableMoFusion(Ours) &- & \textcolor{red}{$0.155^{\pm0.079}$} & \textcolor{blue}{$0.431^{\pm0.003}$} & \textcolor{red}{$0.671^{\pm0.001}$} & \textcolor{red}{$0.789^{\pm0.002}$} & \textcolor{blue}{$10.902^{\pm0.045}$} \\ \hline
% \end{tabular}
% }
% \caption{Quantitative results on the KIT-ML test set. \textcolor{red}{Red} and \textcolor{blue}{Blue} indicate the best and the second best result. The right arrow $\rightarrow$ means the closer to real motion the better. Our method has achieved accuracy improvements on two baseline. Red and Blue indicate the best and the second best result. Our method has achieved accuracy (FID$\downarrow$) improvements on two baseline. }
% % \label{table:kit_ml_results}
% \label{table:kit_ml_results}
% \end{table*}

\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccc}
\hline
\textbf{Method} & \textbf{Venue} & \textbf{FID $\downarrow$} & \multicolumn{3}{c}{\textbf{R-Precision $\uparrow$}} & \textbf{Diversity $\rightarrow$} \\ \cline{4-6}
 & &  & \textbf{top1} & \textbf{top2} & \textbf{top3} \\ \hline
Real & & $0.031^{\pm0.004}$ & $0.424^{\pm0.005}$ & $0.649^{\pm0.006}$ & $0.779^{\pm0.006}$ & $11.08^{\pm0.097}$ \\

MLD \cite{MLD}& CVPR 2023 &$0.404^{\pm0.027}$ & $0.390^{\pm0.008}$ & $0.609^{\pm0.008}$ & $3.204^{\pm0.027}$ & $10.80^{\pm0.117}$ \\

ReMoDiffuse \cite{remodiffuse} & ICCV 2023&$\textcolor{blue}{0.155^{\pm0.006}}$ & $0.427^{\pm0.014}$ & $0.641^{\pm0.004}$ & $0.765^{\pm0.055}$ & $10.80^{\pm0.105}$ \\
MotionDiffuse \cite{motiondiffuse}& TPAMI 2024 & $1.954^{\pm0.062}$ & $0.417^{\pm0.004}$ & $0.621^{\pm0.004}$ & $0.739^{\pm0.004}$ & $11.100^{\pm0.163}$ \\
% MotionLCM \cite{motionlcm} & ECCV 2024& 0.467^{ \pm 0.012} &$0.502^{\pm0.003}$& \textcolor{blue}{$0.701^{\pm 0.002}$} & \textcolor{red}{$0.803^{\pm 0.002}$}  &$9.3610^{\pm 0.660}$\\
T2M-GPT \cite{T2M-GPT}& CVPR 2023 &
$0.514^{\pm0.029}$ & $0.416^{\pm0.006}$ & $0.627^{\pm0.006}$ & $0.745^{\pm0.006}$ & $10.921^{\pm0.108}$\\

MDM\textsubscript{50steps}(baseline) \cite{MDM}& ICLR 2023 & $0.497^{\pm0.021}$ & $0.164^{\pm0.004}$ & $0.291^{\pm0.004}$ & $0.396^{\pm0.004}$ & $10.847^{\pm0.109}$ \\ 

MDM\textsubscript{1000steps}(baseline) \cite{MDM}& ICLR 2023 & $0.556^{\pm0.0698}$ & $0.322^{\pm0.019}$ & $0.431^{\pm0.013}$ & $0.698^{\pm0.052}$ & $10.73^{\pm0.201}$ \\

StableMoFusion (baseline) \cite{stablemofusion} & ACM MM 2024& $0.258^{\pm0.029}$ & \textcolor{red}{$0.445^{\pm0.006}$} & \textcolor{blue}{$0.660^{\pm0.005}$} & \textcolor{blue}{$0.782^{\pm0.004}$} & \textcolor{red}{$10.936^{\pm0.077}$} \\ \hline

Free-MDM\textsubscript{50steps}(Ours) &- & $0.401^{\pm0.033}$ & $0.382^{\pm0.006}$ & $0.587^{\pm0.006}$ & $0.707^{\pm0.007}$ & $10.733^{\pm0.102}$ \\ 

Free-MDM\textsubscript{1000steps}(Ours) &-& $0.529^{\pm0.036}$ & $0.377^{\pm0.004}$ & $0.579^{\pm0.007}$ & $0.705^{\pm0.006}$ & $10.826^{\pm0.117}$ \\ 

Free-StableMoFusion(Ours) &- & \textcolor{red}{$0.155^{\pm0.079}$} & \textcolor{blue}{$0.431^{\pm0.003}$} & \textcolor{red}{$0.671^{\pm0.001}$} & \textcolor{red}{$0.789^{\pm0.002}$} & \textcolor{blue}{$10.902^{\pm0.045}$} \\ \hline
\end{tabular}%
}
\caption{Quantitative results on the KIT-ML test set. \textcolor{red}{Red} and \textcolor{blue}{Blue} indicate the best and the second best result. The right arrow $\rightarrow$ means the closer to real motion the better. Our method has achieved accuracy improvements on two baseline. Red and Blue indicate the best and the second best result. Our method has achieved accuracy (FID$\downarrow$) improvements on two baseline. }
\label{table:kit_ml_results}
\end{table*}

==> tab/lamda.tex <==
\begin{table}[ht]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lllll}
\hline
$\lambda_1$ & $\lambda_2$ & $\lambda_3$  & FID$\downarrow$  & R-Top3$\uparrow$ \\ \hline
1.0         & 1.0        & 1.0  & 0.431$^{\pm0.004}$    & 0.736$^{\pm0.021}$ \\
1.0         & 1.0        & 0.5  & 0.256$^{\pm0.045}$          & 0.757$^{\pm0.005}$ \\

0.5         & 1.0        & 1.0  &  0.301$^{\pm0.021}$     & 0.728$^{\pm0.003}$ \\

1.0         & 0.5        & 1.0  &   0.471$^{\pm0.201}$     & 0.733$^{\pm0.014}$ \\

1.0         & 1.0        & 0.25  & 0.398$^{\pm0.121}$    & 0.755$^{\pm0.011}$ \\
1.0         & 0.25        & 1.0  & 0.592$^{\pm0.001}$    & 0.701$^{\pm0.022}$ \\
0.25         & 1.0        & 1.0  & 1.134$^{\pm0.117}$    & 0.607$^{\pm0.074}$ \\

\hline
\end{tabular}%
}
\caption{Parameter analysis. $\pm$ indicates a 95\% confidence interval. 
R-Top3 represents R-Precision Top3. The table displays the results of three different parameters for loss.}
\label{tab:parameter_analysis}
\end{table}

==> tab/mask.tex <==
\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccc}
\hline
\textbf{Method} & \textbf{FID $\downarrow$} & \multicolumn{3}{c}{\textbf{R-Precision $\uparrow$}} & \textbf{Diversity $\rightarrow$} \\ \cline{3-5}
 &  & \textbf{top1} & \textbf{top2} & \textbf{top3} \\ \hline


NO-Mask Free-MDM    
& $0.310^{\pm0.040}$ 
& $0.452^{\pm0.007}$ 
& $0.648^{\pm0.006}$ 
& $0.755^{\pm0.005}$ 
& $9.824^{\pm0.101}$ \\ 

Mask Free-MDM   
&  $\mathbf{0.261^{\pm0.043}}$
& $\mathbf{0.466^{\pm0.008}}$ 
    & $\mathbf{0.657^{\pm0.007}}$ 
& $\mathbf{0.757^{\pm0.005}}$
&  $\mathbf{9.666^{\pm0.080}}$ \\ 



No-Mask Free-StableMoFusion   
& $0.103^{\pm0.032}$ & $0.491^{\pm0.006}$ & $0.673^{\pm0.012}$ & $0.769^{\pm0.009}$ & $9.110^{\pm0.088}$
 \\ 
Mask Free-StableMoFusion   
& $\mathbf{0.051^{\pm0.002}}$ & $\mathbf{0.520^{\pm0.003}}$ & $\mathbf{0.707^{\pm0.003}}$ & $\mathbf{0.803^{\pm0.006}}$ & $\mathbf{9.480^{\pm0.005}}$\\
\hline
\end{tabular}%
}
\caption{Mask strategy ablation. $\pm$ indicates a 95\% confidence interval. Bold text highlights superior results. Across different baselines, the mask strategy can improve model performance, demonstrating the necessity of applying two distinct consistencies during the denoising stages.}
\label{table:mask_ablation}
\end{table*}

==> tab/rubust.tex <==
\begin{table}[t]
\centering
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{lcc}
\hline
\textbf{Method} & \textbf{FID $\downarrow$} & \textbf{Top-3} \\ \hline

\textbf{MDM}    
& $0.713^{\pm0.023}$ 

& $0.676^{\pm0.006}$ 
 \\ 

\textbf{MDM (Ours)}   
&  $0.467^{\pm0.080}$

& $0.682^{\pm0.004}$
 \\ 

\textbf{Stable MoFusion}   
& $0.202^{\pm0.050}$ 
 
& $0.660^{\pm0.006}$ 

 \\ 

\textbf{Stable MoFusion (Ours)}   
& $0.165^{\pm0.046}$ 
 
 
& $0.703^{\pm0.005}$ 
 \\

\hline
\end{tabular}%
}
\caption{Comparison of robustness testing for MDM and StableMoFusion across different metrics (FID, R-Precision) on the test set.}
\label{table:robustness_test}

\end{table}
% \vspace{-0.5cm}
% \begin{table*}[htbp]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccccc}
% \hline
% \textbf{Method} & \textbf{FID $\downarrow$} & \multicolumn{3}{c}{\textbf{R-Precision $\uparrow$}} & \textbf{Diversity $\rightarrow$} \\ \cline{3-5}
%  &  & \textbf{top1} & \textbf{top2} & \textbf{top3} \\ \hline

% \textbf{MDM}    
% & $0.7132^{\pm0.0231}$ 
% & $0.3218^{\pm0.0032}$ 
% & $0.5121^{\pm0.0039}$ 
% & $0.6763^{\pm0.0061}$ 
% & $9.5632^{\pm0.0055}$ \\ 

% \textbf{MDM (Ours)}   
% &  $0.4677^{\pm0.0802}$
% & $0.3559^{\pm0.0042}$ 
%     & $0.5248^{\pm0.0047}$ 
% & $0.6220^{\pm0.0042}$
% &  $9.4376^{\pm0.0742}$ \\ 

% \textbf{Stable MoFusion}   
% & $0.2020^{\pm0.0500}$ 
% & $0.3998^{\pm0.0048}$ 
% & $0.5683^{\pm0.0051}$ 
% & $0.6599^{\pm0.0057}$ 
% & $9.3747^{\pm0.0887}$
%  \\ 

% \textbf{Stable MoFusion (Ours)}   
% & $0.1646^{\pm0.0460}$ 
% & $0.4319^{\pm0.0047}$ 
% & $0.6080^{\pm0.0050}$ 
% & $0.7032^{\pm0.0052}$ 
% & $9.6169^{\pm0.0742}$ \\

% \hline
% \end{tabular}%
% }
% \caption{Comparison of robustness testing for MDM and Stable MoFusion across different metrics (FID, R-Precision, Diversity) on the test set.}
% \label{table:robustness_test}
% \end{table*}
